Transitional Uncertainty with Layered Intermediate Predictions

In this paper, we discuss feature engineering for single-pass uncertainty estimation. For accurate uncertainty estimates, neural networks must extract differences in the feature space that quantify uncertainty. This could be achieved by current single-pass approaches that maintain feature distances between data points as they traverse the network. While initial results are promising, maintaining feature distances within the network representations frequently inhibits information compression and opposes the learning objective. We study this effect theoretically and empirically to arrive at a simple conclusion: preserving feature distances in the output is beneficial when the preserved features contribute to learning the label distribution and act in opposition otherwise. We then propose Transitional Uncertainty with Layered Intermediate Predictions (TULIP) as a simple approach to address the shortcomings of current single-pass estimators. Specifically, we implement feature preservation by extracting features from intermediate representations before information is collapsed by subsequent layers. We refer to the underlying preservation mechanism as transitional feature preservation. We show that TULIP matches or outperforms current single-pass methods on standard benchmarks and in practical settings where these methods are less reliable (imbalances, complex architectures, medical modalities).

==> Sections/Analysis.tex <==
\section{Representational Feature Preservation under Spurious Inputs}
\label{sec:analysis-feature-preservation}

In Section~\ref{sec:theory-overall}, we described the theoretical disadvantages of representational feature preservation and found that RPF can oppose the learning problem when the preserved features are not related to the application objective. In this section, we analyze a common practical scenario of this case in the form of class imbalance. Under strong imbalances, the training set contains less information of the target distribution resulting in a strong performance decline when features are preserved in the output representation. We investigate this relationship with varying severities of imbalance and compare neural networks with and without explicit representational feature preservation.

%Intuitively, enforcing bi-Lipschitz is an attractive solution for uncertainty estimation as both generalization and feature preservation are optimized jointly with the sensitivity and smoothness constraint. However, by enforcing the bi-Lipschitz constraint during training, the model learns distance features in $\mathcal{X}_{ID}$, where distances do not necessarily correlate with the domain probability $p^*(\bf{x} \in \mathcal{X}_{ID})$ or the target distribution $p^*(y|\bf{x}, \bf{x} \in \mathcal{X}_{ID})$. In this section, we study bi-Lipschitz feature extractors in instances where the training and test set have less semantic overlap and contrast to general limited data settings. From our analysis, we derive several important observations: 1) We find that enforcing bi-Lipschitz lowers generalization performance and uncertainty estimation quality in settings with less semantic overlap of training and test distributions; and 2) bi-Lipschitz constraints increase generalization performance and uncertainty estimation quality in settings with high semantic overlap, even when little training data is available.


% As a result, enforcing Equation~\ref{eq:bi-lipschitz} can result in a severe degradation of performance and uncertainty estimation quality. In this section, we study 



%Spactral nromalization with residual connections is used by both SNGP \citep{liu2020simple} and DUE \citep{van2021due}.

\subsection{Experimental Setup}
We investigate RFP in scenarios where the training set is less informative of the full input distribution. As representational preservation methods have no knowledge of information relevance, spurious information is maintained blindly leading to a performance decline. To illustrate the scenario, we artificially introduce class imbalance at different severity levels. We imbalance the dataset as follows: for a certain subset of classes $A \subset \{1, ..., K\}$, we reduce the the number of training samples by 80\% and do not change the number of test samples. For a second subset $B \subset \{1, ..., K\}, A \cap B = \emptyset$, we reduce the number of test samples by 90\% and do not change the number of training samples. As a result, the first subset of classes contains few training samples and a large amount of test samples, while the other set suffers from the opposite problem. The imbalance severity can be adjusted by the number of classes in both imbalanced subsets $A \cup B \subset \{1, ..., K\}$. For simplicity, we keep the same amount of classes in both subsets $A$ and $B$. In Figure~\ref{fig:class-dist}, we show an overview of class distributions at different severity levels. Here, the top and bottom row contain the training and test distribution respectively.

We perform our entire analysis on the CIFAR100 dataset as it represents a challenging benchmark with a large class variety. In addition, the dataset is fully balanced and contains the same class distribution for training and testing. We further implement representational feature preservation with direct spectral normalization in combination with residual layers. All experiments in this section are conducted with a ResNet-18 model.

%first, we consider settings where the training distribution is similar to the target distribution, but fewer training samples are available. Here, the training set contains similar amount of information with respect to the full distribution $X$, but is more challenging due to the lack of samples. 

%Second, we consider a skewed dataset where the training set contains less information of the full input distribution. 

%To illustrate the first scenario, we remove a percentage of training samples from each class uniformly. Thereby, the class distribution remains equivalent while the problem increases in difficulty due to the lack of samples within each class. 



%We imbalance the dataset as follows: we first select a percentage of classes within CIFAR100 to imbalance. For the first half of our imbalanced classes, we reduce the number if training samples per class from 500 to 100 and do not change the number of test samples. For the second half of imbalanced classes, we do not change the number of training samples but reduce the amount of test samples from 100 to 10 samples per class. As a result, each imbalanced class contains either a small amount of training samples with a large amount of test samples or a large amount of training samples with a small amount test samples. We illustrate the class distributions for different percentages of uniformly removed data, or imbalanced classes within Figure~\ref{fig:class-dist}. The top row shows settings where different percentages of data are uniformly removed within the training set. We note, that the class distributions for training and test sets are equivalent for the first scenario. In contrast, the second row shows the class distributions after artificially unbalancing the a different percentage of classes. Here, the class distributions of training and test are inherently different with different severity levels.
  
\begin{figure*}[!ht]
    \begin{center}
        \includegraphics[scale=0.5]{Fig/class-dist-analysis.png}
    \end{center}
    \caption{Toy example of class distributions at different imbalance severity levels. Each column represents a different severity level, and each column the training and test set distribution respectively.}
    \label{fig:class-dist}
\end{figure*}
\subsection{Classification Accuracy}
We compare the classification accuracy of a standard ResNet-18 architecture with and without spectral normalization in Figure~\ref{fig:acc-analysis}. In addition to our setup on class imbalance, the left graph presents our experiments when both training and test set have the same class distribution with uniformely removed data - i.e. we remove a percentage of random training samples for each class. In contrast to the imbalance scenario, the training set contains similar amount of information with respect to the full distribution $X$, but is more challenging due to the lack of samples. We perform this experiment to show that the performance gain/loss caused by representational feature preservation depends on the available information within the training set, not the number of samples. The right graph shows the imbalanced scenario at different severity levels. Within the left graph, the x-axis shows the amount of uniformly removed training samples in percent; the x-axis on the right represents the fraction of classes that are imbalanced $\frac{|A \cup B|}{K}$. The zero point on the x-axis is equivalent for both scenarios and represents the standard CIFAR100 benchmark without imbalance or data removal. 

Our experiments highlight both advantages and disadvantages of representational feature preservation: if the target distribution is sufficiently similar to the input distribution, additional preserved features correlate with the generalization objective and results in a performance increase - i.e. both $I(h_w(X); Y)$ and $I(h_w(X); X)$ are increased jointly through RFP. From the left graph in Figure~\ref{fig:acc-analysis}, we even gather that gains from representational feature preservation are not subject to the training set size. In fact, the performance gain remains near constant with up to 70\% of the original training data. In contrast, the right graph shows the opposite behavior. Enforcing representational feature preservation results in a strong generalization decline with an approximately 15\% accuracy gap when all 100 classes are unbalanced. In this scenario, the training set contains significantly more information of underrepresented classes in the test set and contains little information of relevant well represented test classes. As spectral normalization preserves features from the training set blindly, spurious information is maintained and results in a performance decline for higher severity levels. Using our previous notation, spectral normalization is increasing $I(h_w(X); X)$ without contributing to $I(h_w(X); Y)$; a direct opposition to the learning objective of neural networks.

%Our results indicate a disadvantage of preserving features under strong distributional shifts: preserved features are less correlated with the target distribution resulting in a performance decline.
\begin{figure*}[!ht]
    \begin{center}
        \includegraphics[scale=0.4]{Fig/acc-spectral-norm.png}
    \end{center}
    \caption{Classification accuracy of a ResNet-18 architecture with and without spectral normalization. We consider two scenarios: a) uniformely removed training and test data (left); and b) class imbalance at different severity levels (right). In both graphs, we show the classification accuracy on the y-axis. The x-axis on the right graph represents the percentage of uniformely removed data, on the left the axis represents the fraction of imbalanced classes.}
    \label{fig:acc-analysis}
\end{figure*}

\subsection{Uncertainty Surface Plots}
In Figure~\ref{fig:surface-plots}, we compare uncertainty estimation capabilities of architectures with and without spectral normalization. In order to generate the plots, we consider a grid of bins over both imbalance severity and uncertainty score. We partition the uncertainty scores for each severity level in ten bins and plot the average test accuracy (top) and number of samples (bottom) for each bin. Considering accuracy vs. uncertainty score provides insights on the uncertainty estimation quality \citep{guo2017calibration}. For high quality estimates, the uncertainty score reflects the classification performance and the relationship between uncertainty and accuracy is linear. Further evaluating the number of samples provides insights on the generalization performance. If the model generalized well to the full input distribution, the number of samples for bins with high accuracy is also high and vice versa.

Within all plots, the x-axis shows the number of imbalanced classes $|A \cup B|$, and the y-axis shows the uncertainty score in predictive softmax entropy. Further, the z-axis shows the test set accuracy in the top row and the number of samples for each bin in the bottom row. From the first row, we see that a conventional neural networks tends to produce overconfident uncertainty scores, regardless of the number of imbalanced classes: for samples with low uncertainty the accuracy is high, but drops near exponentially with higher scores. In other words, the uncertainty score fails to reflect the true accuracy in the model. In contrast, we note that spectral normalization produces a more linear dependency between uncertainty scores and sample accuracy, indicating a higher score quality even with a large quantile of imbalanced classes.  While the uncertainty score quality remains similar, we note that the sample concentration plots indicate a decline in generalization with increasing imbalance severity. For a conventional neural network, most samples are consistently within the bin of the highest accuracy. In contrast, spectral normalization results in a trend inversion with higher class imbalance: samples concentrate in high accuracy bins for low class imbalance and in low accuracy bins for high class imbalance. Our results complement our previous analysis of Figure~\ref{fig:acc-analysis} and indicate the preservation of spurious features when the training set contains less information of the full input distribution.

%In contrast to accuracy, the sample concentration depicts the number of samples within each bin with respect to uncertainty score or dataset imbalance. Within a conventional neural network the majority of samples are concentrated in areas of high accuracy indicating a consistent generalization performance. With spectral normalization, the sample concentration is inverted: for low data imbalance the sample majority is concentrated in low uncertainty and high accuracy bins. For high data imbalance, the samples are concentrated in high uncertainty values with low accuracy. Complementary to Figure~\ref{fig:acc-analysis}, we note a clear generalization performance decline for bi-Lipschitz extractors under distributional shift, but note favorable calibration performance. 
\begin{figure*}[!ht]
    \begin{center}
        \includegraphics[scale=0.4]{Fig/spectral-vs-dnn-surface.png}
    \end{center}
    \caption{Accuracy and number of samples (sample concentration) with respect to dataset imbalance and average uncertainty score. In the the top row we show accuracy, in the bottom row we show sample concentration. The left column represents a conventional DNN while the right shows representational feature preservation through spectral normalization.}
    \label{fig:surface-plots}
\end{figure*}

%\subsection{Misprediction Detection}
%We further benchmark bi-Lipschitz feature extractors within the context of misprediction detection (Figure~FIXME!!!!). Similar to our analysis on classification accuracy, we compare a resnet-18 architecture trained with and without a bi-Lipschitz constraint in both limited data settings with no class distribution shift, varying distributional shift through class imbalance. Figure~FIXME!!! is of a similar structure as our experiment on classification accuracy: the left graph shows our experiments on limited data where the x-axis presents different percentages of uniformly removed data points. The right graph shows our experiments on distributional shift where the x-axis is the fraction of unbalanced classes with respect to the total 100 classes. The y-axis in both graphs shows the ARUOC scores for misclassification detection based on predictive uncertainty. In our analysis, we measure predictive uncertainty by calculating the softmax entropy for both feature extractors. 

%Overall, we denote complementary observations to the accuracy plots. Bi-Lipschitz constraints are generally useful when the preserved features aid in reducing the loss accrued within the target application. For the left graph, both training and test distributions are similar and feature preservation is helpful in detecting misclassifications. In contrast, the right graph shows a performance decline with increasing distributional shift; a result of preserving features hindering misclassification detection.


==> Tables/imagenet.tex <==
%\begin{tabular}{||p{0.55cm}p{0.25cm}p{0.25cm}p{0.25cm}p{0.25cm}p{0.25cm}p{0.25cm}p{0.55cm}|p{0.50cm}p{0.7cm}||}
\begin{table}
\tiny
\centering
\caption{OOD detection and classification accuracy on the ImageNet dataset.}
\label{tab:imgnet-rn}
%\tiny

%\resizebox{\textwidth}{!} {
\begin{tabular}{l c c c}
\hline
%\begin{tabular}{ccccccccccccccccccc} \hline
              % &           &     &     & \multicolumn{3}{c}{\centering OOD AUROC} \\
              Algorithms & Accuracy & ECE & ImageNet-C \\
		% for xray xmax = 2000
        % for CIFARs xmax = 20000 but 15k gives better results
		\hline
		\hline
        %\cline{2-7}
        DNN                & \multirow{3}{*}{72.617 ± 0.019}       & \multirow{2}{*}{1.138 ± 0.005} & 0.868 ± 0.002    \\
    	Energy-Based       &     &                    & 0.861 ± 0.003      \\
    	MC-Dropout         &     & 0.837 ± 0.000      & 0.877 ± 0.000     \\
        \hline
		\texttt{TULIP}    & 72.617 ± 0.019   & 0.700 ± 0.000 & 0.895 ± 0.000   \\
\end{tabular}
%}

%\end{threeparttable}
\end{table}
